Utility-Fairness Trade-Offs and How to Find Them

When building classification systems with demographic fairness considerations, there are two objectives to satisfy: 1) maximizing utility for the specific task and 2) ensuring fairness w.r.t. a known demographic attribute. These objectives often compete, so optimizing both can lead to a trade-off between utility and fairness. While existing works acknowledge the trade-offs and study their limits, two questions remain unanswered: 1) What are the optimal trade-offs between utility and fairness? and 2) How can we numerically quantify these trade-offs from data for a desired prediction task and demographic attribute of interest? This paper addresses these questions. We introduce two utility-fairness trade-offs: the Data-Space and Label-Space Trade-off. The trade-offs reveal three regions within the utility-fairness plane, delineating what is fully and partially possible and impossible. We propose U-FaTE, a method to numerically quantify the trade-offs for a given prediction task and group fairness definition from data samples. Based on the trade-offs, we introduce a new scheme for evaluating representations. An extensive evaluation of fair representation learning methods and representations from over 1000 pre-trained models revealed that most current approaches are far from the estimated and achievable fairness-utility trade-offs across multiple datasets and prediction tasks.

==> 06-ablation.tex <==
\section{Additional Analysis\label{sec:ablation}}
We present additional analysis on \methodName{} and its ability to find the optimal trade-offs. First, we study the effect of kernel choice on the estimated trade-off. Second, we study the relation between the fairness metrics by estimating the trade-off for one metric but evaluating other metrics.

\begin{figure}[ht!]
    \centering
    \captionsetup[subfigure]{oneside,margin={3em,0em}}
    \begin{subfigure}[c]{0.44\linewidth}
        \centering
        \scalebox{0.49}{
        \input{./plots/abl-folk-eo-linear}
        }
        \caption{}
        \label{fig:abl:linear-kernel}
    \end{subfigure}
    \hspace{1em}
    \begin{subfigure}[c]{0.44\linewidth}
        \centering
        \scalebox{0.49}{
        \input{./plots/abl-folk-eo-util}
        }
        \caption{}
        \label{fig:abl:acc-eo}
    \end{subfigure}    
    \caption{(a) Demonstrates the impact of using the Gaussian kernel in the model in comparison to the linear kernel. (b) compares obtained accuracy versus EOD trade-offs of two models that one of them is optimized for EO and the other one is optimized for EOO. 
    \label{fig:abl}}
\end{figure}

\noindent\textbf{Impact of the kernel:} 
In \cref{fig:abl:linear-kernel}, we compare the performance of our method with a Gaussian kernel to that with a linear kernel on the FolkTables dataset. The figure shows that while the linear kernel can closely match the performance of the Gaussian kernel, it is less stable and loses accuracy at higher EOD levels compared to the Gaussian kernel.

\noindent\textbf{Impact of the definition of fairness:}
In this experiment, we're exploring how optimizing our method, \methodName, for a different fairness metric affects the trade-off between accuracy and fairness. We compare two scenarios: one where we optimize for EOD and another for EOOD. We call these methods \methodName-EO and \methodName-EOO, respectively. The results in \cref{fig:abl:acc-eo} show that \methodName-EO achieves higher accuracy than \methodName-EOO at a fixed EOD value. This difference is because \methodName-EOO must satisfy an additional fairness condition for both positive and negative outcomes, which leads to some loss of target attribute information.

